Thermodynamic Properties of Holographic Multiquark and the Multiquark Star

We study thermodynamic properties of the multiquark nuclear matter. The dependence of the equation of state on the colour charges is explored both analytically and numerically in the limits where the baryon density is small and large at fixed temperature between the gluon deconfinement and chiral symmetry restoration. The gravitational stability of the hypothetical multiquark stars are discussed using the Tolman-Oppenheimer-Volkoff equation. Since the equations of state of the multiquarks can be well approximated by different power laws for small and large density, the content of the multiquark stars has the core and crust structure. We found that most of the mass of the star comes from the crust region where the density is relatively small. The mass limit of the multiquark star is determined as well as its relation to the star radius. For typical energy density scale of $10\text{GeV}/\text{fm}^{3}$, the converging mass and radius of the hypothetical multiquark star in the limit of large central density are approximately $2.6-3.9$ solar mass and 15-27 km. The adiabatic index and sound speed distributions of the multiquark matter in the star are also calculated and discussed. The sound speed never exceeds the speed of light and the multiquark matters are thus compressible even at high density and pressure.

==> test.tex <==
It is known that the spherical symmetric dense star has metric in the form
\begin{equation}
ds^{2}=\left( 1-\frac A^{*}( r)dt^{2}
\end{equation}


